Embedding Adaptation is Still Needed for Few-Shot Learning

Constructing new and more challenging tasksets is a fruitful methodology to analyse and understand few-shot classification methods. Unfortunately, existing approaches to building those tasksets are somewhat unsatisfactory: they either assume train and test task distributions to be identical -- which leads to overly optimistic evaluations -- or take a "worst-case" philosophy -- which typically requires additional human labor such as obtaining semantic class relationships. We propose ATG, a principled clustering method to defining train and test tasksets without additional human knowledge. ATG models train and test task distributions while requiring them to share a predefined amount of information. We empirically demonstrate the effectiveness of ATG in generating tasksets that are easier, in-between, or harder than existing benchmarks, including those that rely on semantic information. Finally, we leverage our generated tasksets to shed a new light on few-shot classification: gradient-based methods -- previously believed to underperform -- can outperform metric-based ones when transfer is most challenging.

==> results/table_ood_comparison.tex <==
% !TEX root = ../main_cvpr2021.tex

\begin{table*}[h]
\vspace{0em}
\centering
\caption{
    Comparison of our splits against OOD datasets.
    Our class splits are of similar transfer difficulty to OOD datasets. ($W \approx Y$)
    Because our train classes are more similar, they also make transferring to OOD more difficult. ($Y \geq V$)
}
\label{tOODCompare}
\setlength{\tabcolsep}{3pt}
{\small
\begin{tabular}{l cc c cc}
\addlinespace
\toprule
Source \rarrow  & \multicolumn{2}{c}{mini-ImageNet} &        & \multicolumn{2}{c}{tiered-ImageNet} \\
\cmidrule{2-3} \cmidrule{5-6}

Target \darrow & Original Splits & Our Splits &  & Original Splits & Our Splits \\
\midrule
Test Classes   & XX.X\%          & WW.W\%     &  & XX.X\%          & WW.W\%  \\
\midrule
CUB200         & YY.Y\%          & VV.V\%     &  & YY.Y\%          & VV.V\%  \\
Airplanes      & YY.Y\%          & VV.V\%     &  & YY.Y\%          & VV.V\%  \\
Textures       & YY.Y\%          & VV.V\%     &  & YY.Y\%          & VV.V\%  \\
Quickdraw      & YY.Y\%          & VV.V\%     &  & YY.Y\%          & VV.V\%  \\

\bottomrule
\end{tabular}
}
\vspace{0em}
\end{table*}


